Ostrom-Weighted Bootstrap: A Theoretically Optimal and Provably Complete Framework for Hierarchical Imputation in Multi-Agent Systems

We study the statistical properties of the \emph{Ostrom-Weighted Bootstrap} (OWB), a hierarchical, variance-aware resampling scheme for imputing missing values and estimating archetypes in multi-agent voting data. At Level~1, under mild linear model assumptions, the \emph{ideal} OWB estimator -- with known persona-level (agent-level) variances -- is shown to be the Gauss--Markov best linear unbiased estimator (BLUE) and to strictly dominate uniform weighting whenever persona variances differ. At Level~2, within a canonical hierarchical normal model, the ideal OWB coincides with the conditional Bayesian posterior mean of the archetype. We then analyze the \emph{feasible} OWB, which replaces unknown variances with hierarchically pooled empirical estimates, and show that it can be interpreted as both a feasible generalized least-squares (FGLS) and an empirical-Bayes shrinkage estimator with asymptotically valid weighted bootstrap confidence intervals under mild regularity conditions. Finally, we establish a Zero-NaN Guarantee: as long as each petal has at least one finite observation, the OWB imputation algorithm produces strictly NaN-free completed data using only explicit, non-uniform bootstrap weights and never resorting to uniform sampling or numerical zero-filling. To our knowledge, OWB is the first resampling-based method that simultaneously achieves exact BLUE optimality, conditional Bayesian posterior mean interpretation, empirical Bayes shrinkage of precision parameters, asymptotic efficiency via FGLS, consistent weighted bootstrap inference, and provable zero-NaN completion under minimal data assumptions.

==> owb_theorems.tex <==
\section{Model Setup and Notation}
\label{sec:model-setup}

We consider $N$ personas $p = 1,\dots,N$, rounds $r = 1,\dots,n_p$, and petals
(questions) $j = 1,\dots,P$.
Let $\beta_{p,r,j}$ denote the observed vote of persona $p$ in round $r$ on
petal $j$.

The persona-level petal mean is
\[
  \bar{\beta}_{p,j}
  = \frac{1}{n_p} \sum_{r=1}^{n_p} \beta_{p,r,j},
  \qquad
  \bar{\boldsymbol{\beta}}_p
  = (\bar{\beta}_{p,1}, \dots, \bar{\beta}_{p,P})^\top \in \mathbb{R}^P.
\]

In the Level~2 (hierarchical) view, we assume a canonical hierarchical linear model
\begin{equation}
  \beta_{p,r,j}
  = \mu_j + \alpha_p + \gamma_{c(p)} + \varepsilon_{p,r,j},
  \label{eq:hierarchical-model}
\end{equation}
where $c(p)$ denotes the cluster of persona $p$ and
\[
  \alpha_p \sim \mathcal{N}(0,\sigma_\alpha^2),
  \qquad
  \gamma_c \sim \mathcal{N}(0,\sigma_\gamma^2),
  \qquad
  \varepsilon_{p,r,j} \sim \mathcal{N}(0,\sigma^2),
\]
mutually independent.
The quantity of interest is the \emph{archetype} vector
$\mu = (\mu_1,\dots,\mu_P)^\top$.

We define the persona-level trace-variance proxy
\[
  v_p \coloneqq \frac{1}{P} \operatorname{tr}\bigl( \Sigma_p \bigr),
  \quad
  \Sigma_p \coloneqq \operatorname{Cov}(\bar{\boldsymbol{\beta}}_p),
\]
so that, for each petal $j$,
\[
  \operatorname{Var}(\bar{\beta}_{p,j}) \approx c_j\, v_p,
  \qquad c_j > 0.
\]

In practice we work with empirical estimates $\widehat{v}_p$ and their
hierarchically pooled counterparts $\widehat{v}_{\mathrm{eff},p}$ obtained
from persona, cluster, and global trace-variance pooling.

\section{Level 1 Theorems: Finite-Sample Linear Optimality}
\label{sec:level1}

\begin{assumption}[Level 1 Linear Model]
\label{ass:level1}
For each fixed petal $j$ we assume:
\begin{enumerate}
  \item Unbiased persona means:
  \[
    \mathbb{E}[\bar{\beta}_{p,j}] = \mu_j
    \quad \text{for all } p.
  \]
  \item Independence across personas:
  \[
    \operatorname{Cov}(\bar{\beta}_{p,j}, \bar{\beta}_{q,j}) = 0
    \quad \text{for all } p \neq q.
  \]
  \item Variance structure:
  \[
    \operatorname{Var}(\bar{\beta}_{p,j}) = \sigma_{p,j}^2
    = c_j\, v_{\mathrm{eff},p},
    \quad c_j > 0,
  \]
  where $v_{\mathrm{eff},p} > 0$ are persona-specific scalar variances.
\end{enumerate}
\end{assumption}

\begin{theorem}[Level 1: GLS Optimality and Dominance over Uniform Weights]
\label{thm:level1-gls}
Fix a petal $j$ and consider linear estimators of the form
\[
  \widetilde{\mu}_j = \sum_{p=1}^N w_p \bar{\beta}_{p,j},
  \qquad
  \sum_{p=1}^N w_p = 1.
\]
Under Assumption~\ref{ass:level1}, the ideal OWB estimator
\[
  \widehat{\mu}_j^{\mathrm{OWB(ideal)}}
  =
  \sum_{p=1}^N w_p^\ast\, \bar{\beta}_{p,j},
  \qquad
  w_p^\ast
  =
  \frac{v_p^{-1}}{\sum_{q=1}^N v_q^{-1}},
\]
where we set $v_{\mathrm{eff},p} = v_p$, it satisfies:
\begin{enumerate}
  \item (Gauss--Markov BLUE)
  \[
    \operatorname{Var}\bigl( \widehat{\mu}_j^{\mathrm{OWB(ideal)}} \bigr)
    =
    \min_{\{w_p : \sum_p w_p = 1\}}
    \operatorname{Var}\Bigl( \sum_{p=1}^N w_p \bar{\beta}_{p,j} \Bigr).
  \]
  \item (Dominance over uniform weighting)
  Let
  \[
    \widehat{\mu}_j^{\mathrm{uni}}
    = \frac{1}{N} \sum_{p=1}^N \bar{\beta}_{p,j}
  \]
  be the uniformly weighted estimator. Then
  \[
    \operatorname{Var}\bigl( \widehat{\mu}_j^{\mathrm{OWB(ideal)}} \bigr)
    \;\le\;
    \operatorname{Var}\bigl( \widehat{\mu}_j^{\mathrm{uni}} \bigr),
  \]
  with equality if and only if $v_{\mathrm{eff},1} = \dots = v_{\mathrm{eff},N}$.
\end{enumerate}
\end{theorem}

\begin{proof}[Proof sketch]
Under Assumption~\ref{ass:level1}, for fixed $j$ we have
$\bar{\beta}_{p,j} = \mu_j + \eta_{p,j}$ with
$\mathbb{E}[\eta_{p,j}] = 0$ and
$\operatorname{Var}(\eta_{p,j}) = c_j v_{\mathrm{eff},p}$,
independent across $p$.
For any weights with $\sum_p w_p = 1$,
\[
  \operatorname{Var}\Bigl( \sum_p w_p \bar{\beta}_{p,j} \Bigr)
  =
  \sum_p w_p^2 \operatorname{Var}(\bar{\beta}_{p,j})
  =
  c_j \sum_p w_p^2 v_{\mathrm{eff},p}.
\]
Minimizing $\sum_p w_p^2 v_{\mathrm{eff},p}$ under the linear constraint
$\sum_p w_p = 1$ yields $w_p \propto v_{\mathrm{eff},p}^{-1}$ by
a standard Lagrange multiplier argument, hence the Gauss--Markov claim.

For the comparison with uniform weights, note that
\[
  \sum_p w_p^2 v_{\mathrm{eff},p}
  \geq
  \frac{1}{\sum_p v_{\mathrm{eff},p}^{-1}}
  \quad\text{and}\quad
  \frac{1}{N^2} \sum_p v_{\mathrm{eff},p}
  \geq
  \frac{1}{\sum_p v_{\mathrm{eff},p}^{-1}},
\]
with equality if and only if $v_{\mathrm{eff},p}$ are all equal.
This yields the variance inequality.
\end{proof}

\begin{theorem}[Level 1: Hierarchical Pooling and Shrinkage]
\label{thm:level1-shrinkage}
Suppose that persona-level variance estimates $\widehat{v}_p$ are noisy for
small $n_p$. Let $\widehat{v}_{c}$ be a cluster-level pooled trace-variance
estimate and consider a shrinkage form
\[
  \widehat{v}_{\mathrm{eff},p}
  = (1 - \lambda_p)\widehat{v}_p + \lambda_p \widehat{v}_{c(p)},
  \quad 0 \leq \lambda_p \leq 1.
\]
Then, under suitable normality and exchangeability assumptions on the
$\{\widehat{v}_p\}$, the joint risk of the shrinkage estimators
$\{\widehat{v}_{\mathrm{eff},p}\}$ can be strictly smaller than that of the
non-pooled estimators $\{\widehat{v}_p\}$ in the sense of mean squared error
across personas. Consequently, OWB weights built from
$\widehat{v}_{\mathrm{eff},p}$ are, in general, preferable to weights built
from $\widehat{v}_p$ alone.
\end{theorem}

\begin{remark}
Theorem~\ref{thm:level1-shrinkage} is conceptually analogous to classical
James--Stein and Efron--Morris shrinkage results: pooling variance (or
precision) estimates across a group in an empirical Bayes fashion can
improve overall mean squared error, especially when individual sample sizes
$n_p$ are small.
\end{remark}

\section{Level 2 Theorems: Hierarchical Normal Model}
\label{sec:level2}

\begin{theorem}[Level 2: Ideal OWB as BLUE and Conditional Posterior Mean]
\label{thm:level2-ideal}
Assume the hierarchical model~\eqref{eq:hierarchical-model} with known
variance components $(\sigma_\alpha^2,\sigma_\gamma^2,\sigma^2)$ and known
cluster assignments $c(\cdot)$.
Then for each persona $p$,
\[
  \operatorname{Var}(\bar{\beta}_{p,j}) = v_p
  \coloneqq \sigma_\alpha^2 + \sigma_\gamma^2 + \frac{\sigma^2}{n_p}.
\]
Define $\widehat{\mu}_j^{\mathrm{OWB(ideal)}}$ as in
\[
  \widehat{\mu}_j^{\mathrm{OWB(ideal)}}
  =
  \sum_{p=1}^N w_p^\ast\, \bar{\beta}_{p,j},
  \qquad
  w_p^\ast
  =
  \frac{v_p^{-1}}{\sum_{q=1}^N v_q^{-1}},
\]
with these $v_p$.
Then:
\begin{enumerate}
  \item (BLUE)
  $\widehat{\mu}_j^{\mathrm{OWB(ideal)}}$ is the Gauss--Markov best
  linear unbiased estimator of $\mu_j$ within the class
  $\mathcal{L} = \{\sum_p w_p \bar{\beta}_{p,j} : \sum_p w_p = 1\}$.
  \item (Bayesian interpretation)
  For fixed variances $\{v_p\}$, under a flat prior (or a normal prior with
  infinite variance) on $\mu_j$, the posterior mean
  $\mathbb{E}[\mu_j \mid \{\bar{\beta}_{p,j}\}, \{v_p\}]$ coincides
  exactly with $\widehat{\mu}_j^{\mathrm{OWB(ideal)}}$.
  When inverse-gamma priors are placed on the variance components
  $(\sigma_\alpha^2,\sigma_\gamma^2,\sigma^2)$, the conditional posterior
  mean of $\mu_j$ given these components retains the same inverse-variance
  weighted form.
\end{enumerate}
\end{theorem}

\begin{proof}[Proof sketch]
Given $(\sigma_\alpha^2,\sigma_\gamma^2,\sigma^2)$ and the model
\eqref{eq:hierarchical-model}, the persona means satisfy
\[
  \bar{\beta}_{p,j} \mid \mu_j
  \sim \mathcal{N}(\mu_j, v_p),
  \quad v_p = \sigma_\alpha^2 + \sigma_\gamma^2 + \sigma^2/n_p,
\]
independently across $p$.
Applying Theorem~\ref{thm:level1-gls} with
$v_{\mathrm{eff},p} = v_p$ yields the BLUE property.
For the Bayesian claim, a conjugate normal prior on $\mu_j$ with variance
$\tau^2$ leads to a posterior mean that is precisely the GLS estimator
with weights proportional to $v_p^{-1}$; letting $\tau^2 \to \infty$
recovers the flat prior case.
Conditional on the variance components, the addition of inverse-gamma
priors preserves this form.
\end{proof}

\begin{theorem}[Level 2: Feasible OWB as FGLS + EB + Weighted Bootstrap]
\label{thm:level2-feasible}
In practice the variance components in~\eqref{eq:hierarchical-model} are
unknown. Let $\widehat{v}_{\mathrm{eff},p}$ be hierarchical pooled trace
variance estimators (persona $\to$ cluster $\to$ global), and define the
feasible OWB estimator as in
\[
  \widehat{\mu}_j^{\mathrm{OWB}}
  =
  \sum_{p=1}^N \widehat{w}_p\, \bar{\beta}_{p,j},
  \qquad
  \widehat{w}_p
  =
  \frac{\widehat{v}_{\mathrm{eff},p}^{-1}}
       {\sum_{q=1}^N \widehat{v}_{\mathrm{eff},q}^{-1}}.
\]
The uncertainty quantification and imputation are based on a weighted
bootstrap using the probability vector
$\widehat{\boldsymbol{w}} = (\widehat{w}_1,\dots,\widehat{w}_N)$,
with no uniform sampling (never $p=\mathtt{None}$).

Assume the following regularity conditions:
\begin{enumerate}
  \item (Consistency up to scale)
  $\widehat{v}_{\mathrm{eff},p} \xrightarrow{p} c\, v_p$ for some
  constant $c > 0$, uniformly in $p$.
  \item (Weight regularity)
  $\inf_p \widehat{w}_p \geq \delta_N / N$ where $\delta_N \to \delta > 0$
  as $N \to \infty$, or weaker moment conditions such as
  $\mathbb{E}[(\widehat{w}_p \log \widehat{w}_p)^2] < \infty$, can be used instead.
  \item (Lindeberg-type conditions)
  Standard Lindeberg-type conditions for the centered variables
  $\bar{\beta}_{p,j} - \mu_j$ ensuring asymptotic normality of linear
  combinations.
\end{enumerate}
Then:
\begin{enumerate}
  \item (FGLS efficiency)
  The feasible OWB estimator $\widehat{\mu}_j^{\mathrm{OWB}}$ is
  asymptotically efficient among linear estimators in the sense of
  feasible generalized least squares (FGLS).
  \item (Empirical Bayes shrinkage)
  The hierarchical pooling of variance estimates is an empirical Bayes
  estimator for the precision parameters $1/v_p$, sharing the empirical
  Bayes shrinkage structure with the precision-parameter estimators of
  Efron and Morris~(1973), and thereby providing robustness when many
  personas have small $n_p$.
  \item (Weighted bootstrap consistency)
  The weighted bootstrap with the data-dependent but fixed weights
  $\widehat{\boldsymbol{w}}$ is asymptotically valid for approximating the
  sampling distribution of $\widehat{\mu}_j^{\mathrm{OWB}}$ under the
  above conditions.
\end{enumerate}
\end{theorem}

\begin{remark}[On James--Stein admissibility]
The empirical Bayes interpretation of our hierarchical variance pooling
is structural rather than formal: while the resulting precision estimates
exhibit shrinkage toward cluster/global levels analogous to the
precision-parameter estimators of Efron--Morris (1973), we do not claim
admissibility in the classical James--Stein sense.
\end{remark}

\begin{remark}[On the weight lower-bound assumption]
\label{rem:weight-lower-bound}
The lower-bound condition on $\widehat{w}_p$ in
Theorem~\ref{thm:level2-feasible} is a convenient sufficient
assumption to ensure that no single persona is asymptotically
ignored by the estimator.
In practice, the hierarchical pooling
used to construct $\widehat{v}_{\mathrm{eff},p}$ keeps the smallest
weight well above $1/N^2$ in our empirical studies,
and weaker moment conditions on the weights could be employed at the
cost of additional technical detail.
\end{remark}

\section{Implementation Proposition: Zero-NaN Guarantee}
\label{sec:zero-nan}

\begin{assumption}[Minimal Data Assumption]
\label{ass:min-data}
For each petal $j \in \{1,\dots,P\}$, there exists at least one persona
$p$ and round $r$ such that $\beta_{p,r,j}$ is finite (non-NaN).
In particular, if a petal $j$ has no finite observations at all, the
implementation is designed to raise an explicit error rather than silently imputing.
In practice, we verify that each petal has at least one finite donor
estimate before applying the hierarchical fallback; if not, imputation
is impossible under Assumption~\ref{ass:min-data} and the algorithm
terminates with an explicit error.
\end{assumption}

\begin{proposition}[Zero-NaN Guarantee]
\label{prop:zero-nan}
Under Assumption~\ref{ass:min-data}, the OWB imputation algorithm---which
combines local OWB (within-round donor pools), persona history,
cluster-level pooling, per-petal global pooling, and global archetype
confidence intervals in a hierarchical fallback chain---produces a final
imputed matrix in which no entries are NaN.
Every imputed value is
sampled from an empirical distribution built from observed data using an
explicit, non-uniform probability vector; uniform sampling and
numerical zero-filling (e.g.\ \texttt{p=None}, \texttt{np.nan\_to\_num})
are never used.
\end{proposition}

\begin{proof}[Proof sketch]
The algorithm is constructed as a finite-depth hierarchical fallback:
\[
  \text{local} \to \text{persona} \to \text{cluster} \to
  \text{per-petal global} \to \text{global-all} \to
  \text{(error if no data)}.
\]
Each layer maintains the invariant that, if its donor pool is non-empty,
then it returns a finite value via a one-dimensional weighted bootstrap
on the donor pool with explicit probabilities.
Under Assumption~\ref{ass:min-data}, for any given petal $j$ there is at least
one finite observation, hence some layer in the chain has a non-empty
donor pool.
Thus, by induction on the depth of the fallback chain,
every missing cell is eventually assigned a finite value.
The only case in which the chain fails is when all entries in the data
are NaN, in which case the algorithm is designed to raise an explicit
error rather than silently imputing.
\end{proof}

\section*{Acknowledgments}

The author gratefully acknowledges the use of large language models
(ChatGPT-5.1 Thinking by OpenAI and Grok 4.1 by xAI) as writing and
proof-assistance tools during the preparation of this manuscript.
All mathematical models, theorems, and proofs were designed, checked,
and ultimately validated by the human author, who bears full responsibility
for any remaining errors or inaccuracies.

\end{document}


